Fractional Cone Splines and Hex Splines

We introduce an extension of cone splines and box splines to fractional and complex orders. These new families of multivariate splines are defined in the Fourier domain along certain $s$-dimensional meshes and include as special cases the three-directional box splines \cite{article:condat} and hex splines \cite{article:vandeville} previously considered by Condat, Van De Ville et al. These cone and hex splines of fractional and complex order generalize the univariate fractional and complex B-splines defined in \cite{article:ub,article:fbu} and investigated in, e.g., \cite{article:fm,article:mf}. Explicit time domain representations are derived for these splines on $3$-directional meshes. We present some properties of these two multivariate spline families such as recurrence, decay and refinement. Finally it is shown that a bivariate hex spline and its integer lattice translates form a Riesz basis of its linear span.

==> directionalmeshes.tex <==
%
\section{Cone Splines on $3$-Directional Meshes and Hex Splines}
%
We are interested in deriving formulas for bivariate \textit{hex splines}.  These splines are special cases of box splines where the knot set consists of repeated occurrences of the knots $\bx^1$, $\bx^2$, and $-\bx^3$ where $\bx^3 = \bx^1 + \bx^2$, where $\bx^1, \bx^2$ are linearly independent.  The resulting region of support is then a hexagon -- see Figure \ref{fig:hexsplinesupport}.
%
%
\begin{figure}[ht]
%
    \begin{center}
        \resizebox{\textwidth}{!}{\includegraphics{fig3.png}}
    \end{center}
    %
    \caption{Support for hex splines using the knots $\bx^1 = \left(\frac{1}{2}, -\frac{\sqrt{3}}{2}\right)^T$, $\bx^2 = \left(\frac{1}{2}, \frac{\sqrt{3}}{2}\right)^T$, and $-\bx^3 = -\bx^1-\bx^2 = (-1,0)^T$.  The knot sets, left to right, are $\bX = \left\{ \bx^1,\bx^2,-\bx^3\right\}$, $\bX = \left\{ \bx^1,\bx^1, \bx^2,-\bx^3\right\}$, $\bX = \left\{ \bx^1, \bx^2,\bx^2,-\bx^3,-\bx^3\right\}$, and $\bX = \left\{ \bx^1, \bx^1, \bx^2, \bx^2, -\bx^3, -\bx^3\right\}$.}
    %
    \label{fig:hexsplinesupport}
%
\end{figure}
%
Let $\mathbf{n} = \left( n_1, n_2, n_3\right) \in \mathbb{Z}^3_>$ and $\bX = \left\{ \bx^1, \bx^2, \bx^3\right\}$.  We denote the hex spline as
%
\begin{equation*}
    \Bnspline = B\left(\bx \bigr| \left\{ \underbrace{\strut \bx^1, \ldots \bx^1}_{n_1 \ \mbox{\scriptsize{times}}}, \underbrace{\bx^2, \ldots, \bx^2}_{n_2 \ \mbox{\scriptsize{times}}}, \underbrace{-\bx^3, \ldots -\bx^3}_{n_3 \ \mbox{\scriptsize{times}}} \right\}\right)
\end{equation*}
%
and note that using \eqref{boxft}, the Fourier transform of the hex spline is
%
\begin{align}
%
\widehat{B}_{\mathbf{n}}(\bomega \bigr| \bX) &=
     \frac{\left(1-e^{-\langle\bomega, \bx^1\rangle}\right)^{n_1}\left(1-e^{-\langle\bomega, \bx^2\rangle}\right)^{n_2}\left(e^{\langle\bomega, \bx^3\rangle}-1\right)^{n_1}}{\left(i\langle \bomega, \bx^1\rangle\right)^{n_1} \left(i\langle \bomega, \bx^2\rangle\right)^{n_2} \left(i\langle \bomega, \bx^3\rangle\right)^{n_3}} \nonumber \\
     &= \left(1-e^{-\langle\bomega, \bx^1\rangle}\right)^{n_1}\left(1-e^{-\langle\bomega, \bx^2\rangle}\right)^{n_2}\left(e^{\langle\bomega, \bx^3\rangle}-1\right)^{n_1} \widehat{C}_{\mathbb{n}}\left(\bomega \bigr| \left\{ \bx^1, \bx^2, \bx^3\right\}\right). \label{hexsplineft}
%
\end{align}
%
Thus we are interested in finding explicit formulas for cone splines on the so-called \textit{three-directional meshes} $\bX = \left\{ \bx^1, \bx^2, \bx^1 + \bx^2\right\}$.
%

For the special case $\mathbf{n} = \left( n, n, n\right)$, $n \in \mathbb{Z}_>$ and knot set $\bX = \left\{ \bx^1, \bx^2, \bx^3\right\}$ where
%
\begin{equation*}
    \bx^1 = \left(\begin{array}{c} \frac{1}{2} \\ -\frac{\sqrt{3}}{2} \end{array}\right), \qquad \bx^2 = \left(\begin{array}{c} \frac{1}{2} \\ \frac{\sqrt{3}}{2} \end{array}\right), \qquad  \bx^3 = \bx^1 + \bx^2 = \left(\begin{array}{c} 1 \\ 0 \end{array}\right),
%
\end{equation*}
%
Condat and Van De Ville \cite{article:condat} were able to derive a closed formula for $\Cnspline$:
%
\begin{align}
%
    \Cnspline &= \frac{2}{\sqrt{3}}\sum_{k=0}^{n-1} \binom{n-1+k}{k} \frac{1}{(n-1-k)!(2n-1+k)!}  \nonumber \\
        &{}  \qquad\qquad \times \left(\frac{2\lvert x_2\rvert}{\sqrt{3}}\right)^{n-1-k} \left(x_1 - \frac{\lvert x_2\rvert}{\sqrt{3}}\right)_+^{2m-1+k}.         \label{condatcone}
%
\end{align}
%
Let $M = \left[ \bx^1 \bx^2 \right]$.  Rewriting $\left(1-e^{-\langle\bomega, \bx^1\rangle}\right)^m\left(1-e^{-\langle\bomega, \bx^2\rangle}\right)^m\left(e^{\langle\bomega, \bx^3\rangle}-1\right)^m$ as
%
\begin{equation*}
%
    \widehat{s}(\bomega) = \sum_{\mathbf{k} \in \mathbb{Z}^2} c_{k_1,k_2} e^{-ik_1\langle \bomega, \bx^1\rangle} e^{-ik_2\langle \bomega, \bx^2\rangle} \\
        = \sum_{\mathbf{k}\in \mathbb{Z}^2} c_{k_1,k_2} e^{-i\langle M^T\bomega,\mathbf{k}\rangle}
\end{equation*}
%
where
%
\begin{equation}
    c_{k_1,k_2} = \sum_{k=\max\left(k_1,k_2,0\right)}^{\min\left(n+k_1,n+k_2,n\right)} (-1)^{k_1+k_2+k} \binom{n}{k-k_1}\binom{n}{k-k_2}\binom{n}{k},       \label{condatcoeffs}
\end{equation}
%
Condat and Van De Ville were able to show
%
\begin{equation*}
    s(\bx) =\sum_{\mathbf{k}\in\mathbb{Z}^2} c_{k_1,k_2} \delta(\bx - M\mathbf{k}).
\end{equation*}
%
Using \eqref{hexsplineft} gives
%
\begin{equation}
    \Bnspline = s(\bx) * \Cnspline = \sum_{\mathbf{k}\in\mathbb{Z}^2} c_{k_1,k_2} C_{\mathbf{n}}(\bx - M\mathbf{k}).  \label{hexspline}
\end{equation}
%
or, upon simplification,
%
\begin{align}
    \Bnspline &= \sum_{k_1,k_2 = -n}^n c_{k_1,k_2} \sum_{k=0}^{n-1} \binom{n-1+k}{k} \frac{1}{2n-1+k)!(n-1-k)!} \nonumber \\
        & \quad  \times \bigr| \frac{2x_2}{\sqrt{3}} + k_1 - k_2\bigr|^{n-1-k} \left(x_1 - \frac{k_1+k_2}{2} - \bigr| \frac{x_2}{\sqrt{3}} + \frac{k_1-k_2}{2}\bigr|\right)_+^{2n-1+k}.      \label{condatbox}
\end{align}
%
Figure \ref{fig:condatsplines} shows the hex splines of Condat and Van De Ville for $n=1,2$.
%
\begin{figure}[ht]
%
    \begin{center}
        \resizebox{\textwidth}{!}{\includegraphics{fig4.png}}
    \end{center}
    %
    \caption{$\Cnspline$ generator for $\Bnspline$ for $n=1$ (top row) and $n=2$ (bottom row).  The functions in the top row are piecewise linear and the functions on the bottom row are piecewise quartic.}
    %
    \label{fig:condatsplines}
%
\end{figure}
%

It is straightforward to generalize \eqref{condatcone} and \eqref{condatcoeffs} for the case when the knots of $\bX$ are not repeated the same amount of times.  Once this is done, we can use \eqref{hexspline} to obtain an explicit formula for hex splines with ``weight" vectors of the form $\mathbf{n} = \left( n_1, n_2, n_3\right)$.
%

In order to derive a formula similar to \eqref{condatcone} for $\mathbf{n} = \left( n_1, n_2, n_3\right)$, we first need the following result for $s$-dimensional cone splines on $s$-directional meshes.
%
\begin{conesdirection}
%
                \label{prop:conesdirection}
%
Let $\bX = \left\{ \bx^1, \ldots, \bx^s \right\} \subset \mathbb{R}^s$ be a linearly independent set of vectors and suppose $\mathbf{n} = \left( n_1, \ldots, n_s\right) \subset \mathbb{Z}^s_>$.  Then
%
\begin{equation}
%
    \Cnspline = \lvert \det(M)\rvert^{-1} \prod_{k=1}^s \frac{\langle \bx, \bxd^k\rangle_+^{n_k-1}}{\left(n_k-1\right)!}        \label{conespoints}
%
\end{equation}
%
where $M - \left[ \bx^1 \cdots \bx^s \right]$ and $\left\{ \bxd^1, \ldots, \bxd^s\right\}$ is the dual basis to $\bX$.
%
%
\end{conesdirection}
%
\begin{proof}
%
Let $\bE = \left\{ \be^1,\ldots, \be^s\right\}$ be the canonical basis for $\mathbb{R}^s$.  Using \eqref{coneft}, we have
%
\begin{equation*}
    \widehat{C}(\bx \bigr| \bE) = \prod_{k=1}^s \left( \frac{1}{i\langle \bomega, \be^k\rangle} + \pi\delta\left(\langle \bomega, \be^k\rangle\right)\right)
                    = \prod_{k=1}^s \left( \frac{1}{i\omega_k} + \pi\delta\left(\omega_k\right)\right).
\end{equation*}
%
Thus
%
\begin{equation*}
%
    \CnsplineE = \prod_{k=1}^s \int_{\mathbb{R}} \left( \frac{1}{i\omega} + \pi\delta(\omega)\right)^{n_k} e^{i\omega x_k}\diff{\omega}.
%
\end{equation*}
%
But each factor above is simply the $n_k$-fold convolution product $\left(x_k\right)_+^0 * \cdots * \left(x_k\right)_+^0$ and it is easy to establish that this product is $\frac{1}{\left(n_k-1\right)!}\left(x_k\right)_+^{n_k-1}$.  Thus we have
%
\begin{equation*}
    \CnsplineE = \prod_{k=1}^s \frac{\left(x_k\right)_+^{n_k-1}}{\left(n_k-1\right)!}.
\end{equation*}
%
Using \eqref{conerotateknots}, with $A = M$, and the fact that $\Cnspline = C_{\mathbf{n}}\left(\bx \bigr| \left\{ M\be^1,\ldots, M\be^s\right\}\right)$, we can write
%
\begin{equation*}
    \Cnspline = \frac{1}{\lvert\det(M)\rvert} C_{\mathbf{n}}\left(M^{-1}\bx \bigr| \bE\right) \frac{1}{\lvert\det(M)\rvert} \prod_{k=1}^s \frac{\langle \bx, \bxd^k\rangle}{\left(n_k-1\right)!}
\end{equation*}
%
and the proof is complete.
%
\end{proof}
%
We can use Proposition \ref{prop:conesdirection} with $s=2$ to find a closed formula for cone splines whose knot set consists of linearly independent $\bx^1, \bx^2$ and the third knot $\bx^3 = \bx^1 + \bx^2$.  We need the following lemma:
%
\begin{iteratedintegral}
%
    \label{lemma:iteratedintegral}
%
For $n,m,\ell \in \mathbb{Z}_>$ and $x,a,b \in \mathbb{R}$ with $x > a$, let 
%
\begin{equation*}
    F_{(n,m,\ell)}(x,a,b) = \frac{\scz{1}}{\scz{(n-1)!(m-1)!(\ell-1)!}}\int_a^x (u-b)^{n-1}(u-a)^{m-1}(x-u)^{\ell-1}\diff{u}.
\end{equation*}
%
Then
%
\begin{equation*}
    F_{(n,m,\ell)}(x,a,b) = \sum_{k=0}^{n-1} \binom{\scz{m+k-1}}{\scz{k}} \frac{\scz{1}}{\scz{(n-1-k)!(m+\ell+k-1)!}}(b-a)^{n-1-k}(x-a)^{m+\ell+k-1}.
\end{equation*}
%
%
\end{iteratedintegral}
%
\begin{proof}
%
The proof is a straightforward application of Cauchy's formula for repeated integration:
%
\begin{equation}
    \frac{1}{(\ell-1)!} \int_a^x f(t)(x-t)^{\ell-1}\diff{t} = \int_a^x \int_a^{s_1} \cdots \int_a^{s_{\ell-1}} f\left(s_{\ell}\right)\diff{s_{\ell}}\cdots \diff{s_1}.
                \label{cauchyintegral}
\end{equation}
%
We use \eqref{cauchyintegral} with $f(u) = (u-b)^{n-1}(u-a)^{m-1}$ to obtain
%
\begin{align*}
    F_{(n,m,\ell)}(x,a,b) &= \frac{\scz{1}}{\scz{(n-1)!(m-1)!}} \int_a^x \int_a^{s_1} \cdots \int_0^{s_{\ell-1}-a} (u+a-b)^{n-1}u^{m-1}\diff{u}\cdots \diff{s_1} \\
        &= \frac{1}{(n-1)!(m-1)!} \sum_{k=0}^{n-1}\binom{n-1}{k} (a-b)^{n-1-k} \frac{1}{m+k} \\
        &  \qquad \qquad \times \int_a^x \int_a^{s_1} \cdots \int_a^{s_{\ell-2}} \left(s_{\ell-1}-a\right)^{m+k}\diff{s_{\ell-1}}\cdots \diff{s_1}.
\end{align*}
%
Computing the remaining $\ell-1$ integrals gives
%
\begin{align*}
    F_{n,m,\ell)}(x,a,b) &= \frac{\scz{1}}{\scz{(n-1)!(m-1)!}} \sum_{k=0}^{n-1}\binom{\scz{n-1}}{\scz{k}} (a-b)^{n-1-k} \\
        & \qquad \qquad \times \frac{\scz{1}}{\scz{(m+k)\cdots (m+\ell+k-1)}}(x-a)^{m+\ell+k-1} \\
        &= \sum_{k=0}^{n-1} \binom{\scz{m+k-1}}{\scz{k}} \frac{\scz{1}}{\scz{(n-1-k)!(m+\ell+k-1)!}}(a-b)^{n-1-k}(x-a)^{m+\ell+k-1}
\end{align*}
%
Since $x>a$, we can replace $(x-a)$ with $(x-a)_+$ in the last term above and complete the proof.
%
\end{proof}
%
We are now ready to state a closed formula for cone splines on $3$-directional meshes:
%
\begin{cone3direction}
%
    \label{prop:cone3direction}
%
Suppose $\bX \subset \mathbb{R}^2$ is the $3$-directional knot set $\bX = \left\{ \bx^1, \bx^2, \bx^3\right\}$ with $\bx^1, \bx^2$ linearly independent and $\bx^3 = \bx^1 + \bx^2 = (1,0)^T$ and, without loss of generality, $x^1_2 > 0$.  Then the cone spline $\Cnspline$ is given by
%
\begin{equation*}
    \Cnspline = \frac{1}{x^1_2} \left\{ \begin{array}{lll} F_{\left(n_1,n_2,n_3\right)}\left(x_1, \left(\frac{x^1_1}{x^1_2}\right)x_2, \left(\frac{x_1^1-1}{x_2^1}\right)x_2\right), & x_2 \geq 0 \\
                                                 F_{\left(n_2,n_1,n_3\right)}\left(x_1, \left(\frac{x_1^1-1}{x_2^1}\right)x_2, \left(\frac{x^1_1}{x^1_2}\right)x_2\right), & x_2 < 0 
                            \end{array}\right.
\end{equation*}
%
Here, $F$ is given in Lemma \ref{lemma:iteratedintegral}.
%
%
\end{cone3direction}
%
\begin{proof}
%
From \eqref{coneft}, we know that 
%
\begin{equation*}
    \widehat{C}_{\mathbf{n}}(\bomega \bigr| \bX) = \widehat{C}_{\left(n_1,n_2\right)}\left(\bomega \bigr| \left\{ \bx^1, \bx^2\right\}\right) \cdot \left( \frac{1}{i\omega_1} + \pi \delta\left(\omega_1\right)^{n_3}\right)
\end{equation*}
%
so that 
%
\begin{align}
    \Cnspline &= C_{\left(n_1,n_2\right)}\left(\bx \bigr| \left\{\bx^1, \bx^2\right\}\right) * \frac{\left(x_1\right)_+^{n_3-1}}{\left(n_3-1\right)!}\delta\left(x_2\right) \nonumber \\
        &= \left( \vert\det(M)\rvert \prod_{k=1}^3 \left(n_k-1\right)!\right)^{-1} \\
        &  \qquad \qquad \times \int_{-\infty}^{x_1} \langle \left(u,x_2\right), \bxd^1\rangle^{n_1-1}\langle \left(u,x_2\right), \bxd^2\rangle^{n_2-1}\left(x_1-u\right)_+^{n_3-1}\diff{u}
                    \label{coneconvolve}
\end{align}
%
Since $\bx^1 + \bx^2 = (1,0)^T$, we know $\bx^2 = \left( 1-x^1_1, -x^1_2\right)^T$ and from here we can easily show that the dual basis is
%
\begin{equation*}
    \left\{ \bxd^1, \bxd^2\right\} = \left\{ \left( \begin{array}{c} 1 \\ \frac{1-x^1_1}{x^1_2}\end{array}\right), \left(\begin{array}{c} 1 \\ -\frac{x^1_1}{x^1_2}\end{array}\right)\right\} := \left\{ \left( \begin{array}{c} 1 \\ a\end{array}\right), \left( \begin{array}{c} 1 \\ b \end{array}\right)\right\}
\end{equation*}
%
and $\lvert \det(M)\rvert = x^1_2$.  Inserting these identities into \eqref{coneconvolve} and setting $K = \left( x^1_2\prod_{k=1}^3 \left(n_k-1\right)!\right)^{-1}$ gives
%
\begin{align*}
    \Cnspline &= K\int_{-\infty}^{x_1} \left( u - b x_2\right)_+^{n_1-1} 
        \left( u -a x_2\right)_+^{n_2-1}\left(x_1-u\right)^{n_3-1}\diff{u} \\
        &= K \left\{ \begin{array}{ll}
            \int_{a x_2}^{x_1} \left( u - bx_2\right)^{n_1-1}\left( u -a x_2\right)^{n_2-1}\left(x_1-u\right)^{n_3-1}\diff{u}, & x_2 \geq 0 \\
        %
        \int_{b x_2}^{x_1} \left( u - b x_2\right)^{n_1-1}\left( u -a x_2\right)^{n_2-1}\left(x_1-u\right)^{n_3-1}\diff{u}, & x_2 < 0 
        \end{array}\right. .
\end{align*}
%
We can use Lemma \ref{lemma:iteratedintegral} to complete the proof.
\end{proof}
%
\textbf{Remark 1.}  Using \eqref{conerotateknots}, we can easily construct a formula for the cone spline with the general $3$-directional mesh $\bx^1, \bx^2, \bx^1+\bx^2$.
%

\textbf{Remark 2.} Setting $\mathbf{n} = (n,n,n)$ in Proposition \ref{prop:cone3direction} gives the cone spline \eqref{condatcone} of Condat and Van De Ville.
%

We use Proposition \ref{prop:cone3direction} to plot the cone splines shown in Figure \ref{fig:cone3splines}.
%
\begin{figure}[ht]
%
    \begin{center}
        \resizebox{\textwidth}{!}{\includegraphics{fig5.png}}
    \end{center}
    \caption{For $\bX = \left\{ \bx^1,\bx^2,\bx^3\right\}$ where $\bx^1 = \left(\frac{1}{2},\frac{\sqrt{3}}{2}\right)^T$, $\bx^2 = \left(\frac{1}{2},-\frac{\sqrt{3}}{2}\right)^T$ and $\bx^3 = (1,0)^T$, the cone splines plotted left to right are $C_{(1,1,3)}(\bx \bigr| \bX)$, $C_{(2,1,1)}(\bx \bigr| \bX)$, and $C_{(2,3,1)}(\bx \bigr| \bX)$.}
    %
    \label{fig:cone3splines}
%
\end{figure}
%

\begin{itemize}
    %
    \item Proposition for $B_3(x|X)$.
    %
    \item Example
\end{itemize} 

==> fractionalboxsplines.tex <==
%
\section{Fractional Box Splines}
%
\begin{itemize}
    \item Definition.
    %
    \item Proposition for $s$-Directional Meshes.
    %
    \item Example (2D).
    %
    \item Proposition for $3$-directional meshes.
    %
    \item Remark:  Relate to Section 2 result.
    %
    \item Examples
\end{itemize}

==> fractionalconesplines.tex <==
%
\section{Fractional Cone Splines}
%
\begin{itemize}
    \item Definition.
    %
    \item Proposition for $s$-Directional Meshes.
    %
    \item Example.
    %
    \item Proposition - recursion formula.
    %
    \item Proposition for $3$-directional meshes.
    %
    \item Remark:  Relate to Section 2 result.
    %
    \item Examples
\end{itemize}
